Variational Bayesian Inference for Crowdsourcing Predictions

Crowdsourcing has emerged as an effective means for performing a number of machine learning tasks such as annotation and labelling of images and other data sets. In most early settings of crowdsourcing, the task involved classification, that is assigning one of a discrete set of labels to each task. Recently, however, more complex tasks have been attempted including asking crowdsource workers to assign continuous labels, or predictions. In essence, this involves the use of crowdsourcing for function estimation. We are motivated by this problem to drive applications such as collaborative prediction, that is, harnessing the wisdom of the crowd to predict quantities more accurately. To do so, we propose a Bayesian approach aimed specifically at alleviating overfitting, a typical impediment to accurate prediction models in practice. In particular, we develop a variational Bayesian technique for two different worker noise models - one that assumes workers' noises are independent and the other that assumes workers' noises have a latent low-rank structure. Our evaluations on synthetic and real-world datasets demonstrate that these Bayesian approaches perform significantly better than existing non-Bayesian approaches and are thus potentially useful for this class of crowdsourcing problems.

==> conclusion.tex <==
\section{Conclusion}


==> experiment-initial.tex <==
\section{Experimental Results}

\newcommand{\average}{$\mathsf{Average}$}
\newcommand{\indml}{$\mathsf{Ind}$-$\mathsf{ML}$}
\newcommand{\indvb}{$\mathsf{Ind}$-$\mathsf{VB}$}
\newcommand{\latentml}{$\mathsf{Latent}$-$\mathsf{ML}$}
\newcommand{\latentvb}{$\mathsf{Latent}$-$\mathsf{VB}$}

We compare the following five algorithms:
\begin{itemize}
  \item \average\, takes the average of the observed predictions
    as the aggregated value.
  \item \indml\, is the classical inverse variance weighting algorithm that 
    recursively updates ground truth estimates and worker variances 
    using equation~\eqref{eq:ivar}.
  \item \indvb\, is the variational bayes approach
    based on the independent noise model that 
    recursively updates ground truth posteriors and hyperparameters
    using equations~\eqref{eq:ind-vb-truth-var}~--~\eqref{eq:ind-vb-error-param}.
  \item \latentml\, is the inverse covariance weighting algorithm with a
    latent noise feature model that recursively 
    updates ground truth estimates and worker variances using equation~\eqref{eq:icov}
    and performs stochastic gradient descent on the latent features and hyperparameters
    using equation~\eqref{eq:sgd}.
  \item \latentvb\, is the variational bayes approach
    based on the latent noise model that recursively
    updates ground truth and latent posteriors and hyperparameters
    using equations~\eqref{eq:latent-vb-truth-var}~--~\eqref{eq:latent-vb-error-param}.
\end{itemize}

\subsection{Synthetic Datasets}

Motivated by the size and sparsity of the age prediction crowdsource dataset 
(see Section~\ref{sec:real-data}), 
we generate synthetic datasets for $I=1000$ tasks and $J = 500$ workers
with $|J_i| = 10$ workers giving labels for each task.
Since our algorithms are based on two different models,
with significantly different assumptions on worker noises, 
we generate data that includes both model components 
and study the robustness of the algorithms to model misspecification.
Specifically, we use:
\begin{align*}
  x_{ij} 
  = \sigma_y y_i + \sqrt{\alpha}\cdot\epsilon_{ij} + \sqrt{1-\alpha}\cdot\xi_{ij},
\end{align*}
where $\epsilon_{ij}$ and $\xi_{ij}$ are 
independent and latent noise components respectively.
Both components are drawn such that the average variance of each component 
in the system is $1$, and therefore, for all $\alpha\in[0,1]$, 
the total noise variance in the system is $1$. 
The independent noise component is drawn such that 
$\epsilon_{ij} \sim\mathcal{N}(\mathbf{0},\boldsymbol\sigma_j^2)$,
where $\sigma_j^2$ is chosen randomly from the set $\{0.164,1.64,16.4\}$.
The latent noise component is drawn such that $\xi$ is a matrix with rank $D$.
The ground truth values are drawn such that $y_i \sim\mathcal{N}(0,1)$.
Therefore, when $\sigma_y = 1$, the average variance of 
the ground truth and the noise components in the system are equal.

We vary the scaling factor $\sigma_y$ to study 
how the algorithms are affected by 
the noise variance relative to the ground truth variance.
We vary the scaling factor $\alpha$ to study
how the algorithms are affected by
whether the data has a low-rank covariance or diagonal covariance.
All numbers are reported by taking the average of 10 random instances.



\subsection{Human Age Prediction}
\label{sec:real-data}

We compare the performance of the algorithms on a real-world crowdsource dataset
introduced in~\cite{kara2015modeling}. The underlying dataset contains $1002$
pictures of $82$ faces from the $\mathsf{FG}$-$\mathsf{Net}$ database~\cite{FGNet}
in which each photo is labelled with a biological age as the ground truth.
The age of each subject was discretized into $7$ intervals, and $619$
crowdsource workers were asked to classify the age of a subject based on the facial image,
so that each image has $10$ answers from workers.


==> related_work.tex <==
\section{Related work}
%\fbox{Inverse variance weighting literature here}

One of the earliest efforts in prediction aggregation was that of  \cite{dawid1979maximum} who proposed a Bayesian inference algorithm to aggregate individual worker labels and infer the ground-truth  in categorical annotation. Their approach defined the two main components needed in what was later to be known as crowdsource annotation: estimating the reliability of each crowdsource worker, and inferring the true label of each instance.  In their seminal paper,

\cite{dawid1979maximum}
applied expectation maximization and estimated the ground-truth in the E-step. Then, using the
estimated ground-truth, they compute the maximum likelihood estimates of the confusion matrix
in the M-step.

In continuous value annotation, more recently, \cite{raykar2010learning} modeled each worker prediction as an independent noisy observation of the ground-truth. Based on this independent noise assumption, \cite{raykar2010learning} developed a counterpart  to the  Dawid-Skene framework for the continuous domain to infer both the unknown individual variance and the ground-truth.   In their M-step, the variance, which  corresponds to the confusion matrix in categorical annotation, is computed to minimize the mean square error with respect to the estimated ground-truth. Their  E-step involves re-estimating the ground-truth with a weighted sum of the individual predictions, where  the weights are set as  the inverses of individual variances. 
\cite{liu_variational} point to the risk of convergence to a poor-quality local optimum of the above-mentioned EM approaches and propose a variational approach for the problem. 
 \cite{liu2013scoring} took a different tack by injecting  items with ground-truth labels, called control questions, to better estimate the reliability of each crowdsource worker in what they term their "consensus model with partial ground truth".

\cite{NIPS2010_4074}  seek to define groups of behaviors by modeling each crowdsource worker as a multi-dimensional quantity including bias and other factors, and then group them as a function of those quantities.
\cite{kara2015modeling} in a similar vein aim to identify particular types of worker behavior that they wish to model, including bias and 
 the so-called worker opinion scaling.
 
 
Crowdsourcing data  are typically sparse  as the crowdsource workers seldom participate in all of the tasks. This  sparsity  motivates  the application of collaborative filtering and matrix factorization techniques to the crowd-sourcing domain. Along these lines, \cite{zhang2014spectral} proposed a spectral method to  provide an initial estimate of the confusion matrix for EM algorithm. Another application of matrix factorization was proposed by \cite{jung2012improving} to infer the unobserved predictions of workers before applying standard aggregation methods, i.e. majority voting. The above matrix factorization  approaches model the correlation of  errors for  each individual crowdsource worker across instances, as represented by the confusion matrix. 

 However, in many cases, especially the continuous labeling applications such as the medical domain and prediction markets that interest us, crowdsource workers may exhibit correlations in their responses across workers themselves.   \cite{li2019exploiting} showed that the incorporation of cross-worker correlations significantly improves accuracy. Their work, which  focused on  the discrete problem of unsupervised crowdsourced classification, relies on an extension of the (independent) Bayesian Classifier Combination model of \cite{iBCC} in which they model worker correlation by considering that  true classes
are mixtures of subtypes.

Applications in the continuous-label context are often equipped with  ground truth labels on some of the data. This occurs not only when control questions are injected for the purpose of enhancing the model accuracy for each worker, as described by \cite{liu2013scoring}, but also in applications where ground truth is obtained naturally later in time, such as in medical diagnosis and prediction markets.

It is in this context that  \cite{volkovs2012learning}  propose a model to aggregate the rankings of crowdsource workers, or "experts".
They represent the ranking matrix of each  worker by  a low-rank decomposition so as to learn the ranking regression function for the  aggregation.  The supervised framework that they propose is not directly applicable to our setting as  it assumes a fixed set of $K$ crowdsource workers across all instances. In addition, their method of concatenating   experts'  features leads to a model of rather high dimension,  not suitable for the regression tasks that interest us here.
 

